Left-hand cut problem in lattice QCD and an EFT-based solution

Lattice QCD has become an essential tool for studying the hadron-hadron interaction from the first principles. However, when extracting infinite-volume scattering parameters from finite-volume energy levels, the traditional L\"uscher formula encounters limitations due to the left-hand cut induced by long-range interactions such as the one-pion exchange. In this work, we propose an alternative approach based on chiral effective field theory combined with a Hamiltonian method in the plane wave basis. By solving a Schr\"odinger-like equation in the finite volume, our method connects the finite-volume energy spectrum with infinite-volume observables, while systematically incorporating the long-range physics and solving the left-hand cut problem. The use of the plane wave basis mitigates issues related to partial wave mixing. Our numerical results for $DD^*$ scattering at $m_\pi \approx$ 280 MeV demonstrate that this approach overcomes the limitations of the L\"uscher method and points towards a resonance interpretation of the $T_{cc}(3875)$ state, as opposed to the virtual state predicted by traditional analyses.

==> bak.tex <==
% While the irreps $T_1^+(0)$ and $A_2(1)$ can also receive contributions from the 
% $S$-to-$D$-wave short-range interactions as well as from the $^3P_2$ partial waves at ${\cal O}(Q^2)$,  in what follows, we 
% consider  fits with 3-parameters from  Eq.~\eqref{eq:Vct} as our main results and  use the additional contributions from other partial waves to estimate systematic uncertainties in \cite{Suppl_Tcc_EFV}.


% The Lüscher method relates finite-volume energy levels to infinite-volume scattering parameters by assuming that the effects of off-shell contributions are negligible. However, for energies where k² < –mπ²/4, the one-pion exchange produces a left-hand cut that renders the K-matrix complex, thereby complicating the ERE and introducing significant model dependence.






 

 % Following Ref.~\cite{Padmanath:2022cvl}, we consider the nine lowest-lying energy levels in the irreducible representations (irreps) $T_1^+(0), A_1^-(0)$ and $A_2(1)$ of the point groups   as input in our calculations. The integer numbers $d$ in the parentheses are related to  the total momentum of two particles $\bm{P}={2\pi \over L} \bm d$ with $\bm d \in Z^3$. 


 
% \begin{figure*}[t]
% \begin{center}
% \includegraphics[width=0.9\textwidth]{delta_3S1_3P0_CT}
% \includegraphics[width=0.9\textwidth]{delta_3S1_3P0_OPE}
% \caption{\label{fig:phase_shifts}  
% Phase shifts in the $^3S_1$ (left panel) and $^3P_0$ (right panel) partial waves extracted from the FV energy levels $E_{FV}$ calculated in lattice QCD. Red bands represent the results of our 3-parameter fits to  $E_{FV}$
% \emph{without} the OPE (Fit 1, upper panel) and \emph{with} the OPE  (Fit 2, lower panel), including the $1\sigma$ uncertainty.
%    Green dots in the left panel are the  
%  phase shifts extracted from $E_{FV}$ using the single-channel Lüscher quantization conditions in Ref.~\cite{Padmanath:2022cvl}.
%  Green dots in the right panel are extracted in this study using the same method.
% Blue bands are the results of the 4-parameter fits of $E_{FV}$ using the ERE  in   Ref.~\cite{Padmanath:2022cvl}. Orange lines in the left panel correspond to 
% $ip=\pm |p|$ from unitarity,   normalized to $E_{DD^*}$. The gray vertical dashed line denotes the position of the branch point of the left-hand cut nearest to the threshold. } 
% \end{center}
% \end{figure*}
% 


 
% %  \begin{table*}[htp]
% %      \centering
% % \begin{tabular*}{\hsize}{@{}@{\extracolsep{\fill}}lcccccc@{}}
% % \hline 
% % \hline 
% %  & $a_{^{3}\!S_{1}}$ {[}fm{]} & $r_{^{3}\!S_{1}}$ {[}fm{]} & $\delta m_{T_{cc}}$ {[}MeV{]}  & $a_{^{3}\!P_{0}}$ {[}fm$^{3}${]} & $r_{^{3}\!P_{0}}$ {[}fm$^{-1}${]} & $\chi^{2}/\text{dof}$\tabularnewline
% % \hline 

% % LQCs+ERE fit~\cite{Padmanath:2022cvl} & $1.04\pm0.29$ & 0.96$_{-0.20}^{+0.18}$ & $-9.9_{-7.2}^{+3.6}$  & $0.076_{-0.009}^{+0.008}$ & $6.9\pm2.1$ & $3.7/5$\tabularnewline
% %  Fit 1: cont. & $1.09\pm0.35$ & $0.75\pm0.14$ & $-10.6\pm4.4$   & $0.028\pm0.004$ & $-4.3\pm0.05$ & $5.52/6$\tabularnewline
% % Fit 2: cont.+OPE & $1.46\pm0.57$ & $0.096\pm0.53$ & $-6.6(\pm1.5)-i4.0(\pm3.7)$ & $0.497\pm0.007$ & $5.63\pm0.19$ & $2.95/6$\tabularnewline
% % \hline
% % \hline 
% % \end{tabular*}
% %      \caption{\label{tab:ere_pole_num}
% %      Results for the $T_{cc}$ pole position $\delta m_{T_{cc}}$,  defined relative to the $DD^*$ threshold, and the $DD^*$ ERE parameters.
% %      The results obtained via the Lüscher QCs plus ERE in Ref.~\cite{Padmanath:2022cvl} are present in the second row. Our results from  Fits 1 and 2  
% %      are given in the third and forth rows, respectively. 
% %      The   $T_{cc}$ pole position in Fit 2 corresponds to a resonance state with 85\% probability within the $1\sigma$ uncertainty. The residual 
% %      15\% probability corresponds to a scenario with two virtual poles--see the intersection area of the red band with the orange curve in Fig.~\ref{fig:phase_shifts}. 
% %  }  
% %  \end{table*}



% \section{Numerical results}




% \section{Plane wave expansion method}

% Relativistic two-body dynamics can be described in the framework of the Bethe-Salpeter equation. 
% To transform it to a numerically more tractable three-dimensional integral equation, we use the method of Blankenbecler and Sugar equation~\cite{Woloshyn:1973mce}.
 
 
% The Green function reads
% \begin{eqnarray}\label{eq:sm_G_sup}
% G(\bm{q},E)	&=&i\int\frac{dq^{0}}{2\pi}\frac{1}{(P-q)^{2}-m_{1}^{2}+i\epsilon}\frac{1}{q^{2}-m_{2}^{2}+i\epsilon} \nonumber\\
% &=&\frac{1}{4\omega_{1}\omega_{2}} \left(  \frac1{E-\omega_1-\omega_2} - \frac1{E +\omega_1+\omega_2} \right)\nonumber\\
% 	&=&\frac{1}{2\omega_{1}\omega_{2}}\frac{(\omega_{1}+\omega_{2})}{E^{2}-(\omega_{1}+\omega_{2})^{2}+i\epsilon}\,,
% \end{eqnarray}
% with $\omega_{i}=\sqrt{m_{i}^{2}+\bm{q}^{2}}$. Here, the total four-momentum of the two-particle system in the center of mass frame is $P^{\mu}=(E,\bm{0})$, while $q$ and $P-q$ refer to the four-momenta of the particles.  The second line in Eq.~\eqref{eq:sm_G_sup} 
% corresponds to the propagators written in terms of time-ordered perturbation theory (TOPT), with 
% the first term possessing the two-body $DD^*$ cut~\footnote{Neglecting the last term in the second line in Eq.~\eqref{eq:sm_G_sup} corresponds to the Kadyshevsky equation \cite{Kadyshevsky:1967rs} (see also \cite{Baru:2019ndr} for a related discussion). We checked that omitting this term does not have an impact on our results.}.   
% The effects neglected in this treatment start from the so-called stretched boxes -- one loop diagrams in TOPT with no two-body cuts involved and therefore contributing at higher orders, see, e.g.,~\cite{Zhang:2021hcl,Hanhart:2000wf} for a related discussion. 
% The Lippmann-Schwinger-type three-dimensional equation is
% \begin{equation}\label{eq:LSE_supl}
% T(\bm{p},\bm{p}'\!,E)=V(\bm{p},\bm{p}')+\!\int\!\!\frac{d^{3}\bm{q}}{(2\pi)^{3}}V(\bm{p},\bm{q})G(\bm{q},E)T(\bm{q},\bm{p}'\!,E).
% \end{equation}
% The three-dimensional momenta which appear in the equation above are defined in the center of mass frame. 

% For two particles in the FV, the momenta become discrete to satisfy the periodic boundary condition. The quantization condition of momenta in the box frame is $\bm{q}_{n}^{b}=\frac{2\pi}{L}\bm{n}$ with $\bm n\in Z^3$. The total three-dimensional momentum in the box frame is $\bm{P}={2\pi \over L}\bm d$ with $\bm d \in Z^3$. To obtain the LSE in the FV, we replace the integration over the loop momentum  with a summation
% \begin{equation}
%     \int\frac{d^{3}\bm{q}}{(2\pi)^{3}}f(\bm{q})=\int\frac{d^{3}\bm{q}^{b}}{(2\pi)^{3}}{\cal J}f[\bm{q}(\bm{q}^{b})]\to\sum_{\bm{n}\in Z^{3}}\frac{1}{L^{3}}{\cal J}f[\bm{q}(\bm{q}_{n}^{b})],
%     \label{eq:sm_temp_01}
% \end{equation}
% where the Lorentz boost transformation connecting $\bm q$ in the center of mass frame and $\bm q ^b$ in the box frame reads~\cite{Li:2021mob}
% \begin{eqnarray}
%     \bm{q}	&&=\gamma\left(\bm{q}_{\parallel}^{b}-\frac{\omega_{1}^{b}}{\omega_{1}^{b}+\omega_{2}^{b}}\bm{P}\right)+\bm{q}_{\perp}^{b},\\
% \gamma	&&=\frac{\omega_{1}^{b}+\omega_{2}^{b}}{\sqrt{(\omega_{1}^{b}+\omega_{2}^{b})^{2}-\bm{P}^{2}}},
% \end{eqnarray}
% with $\omega_{1}^{b}=\sqrt{m_{1}^{2}+(\bm{q}^{b})^2}$ and $\omega_{2}^{b}=\sqrt{m_{2}+(\bm{P}-\bm{q}^{b})^{2}}$, 
%  $\bm{q}_{\parallel}^{b} =(\bm{q}^{b}\cdot {\bm P}){\bm P}/{\bm P}^2$ and $\bm{q}_{\perp}^{b}=\bm{q}^b-\bm{q}_{\parallel}^{b}$. The Jacobian $\mathcal{J}$ in Eq.~\eqref{eq:sm_temp_01} has the form
% \begin{equation}
%     {\cal J}=\left(\frac{\omega_{1}\omega_{2}}{\omega_{1}+\omega_{2}}\right)\left(\frac{\omega_{1}^{b}\omega_{2}^{b}}{\omega_{1}^{b}+\omega_{2}^{b}}\right)^{-1}.
% \end{equation}
% In FV, the LSE turns into the matrix equation
% \begin{equation}
%     \mathbb{T}=\mathbb{V}+\mathbb{V}.\mathbb{G}.\mathbb{T}\,,
% \end{equation}
% with
% \begin{eqnarray}
% \mathbb{G}(E)=\frac{{\cal J}(\bm{q}_{n})}{L^{3}}G(\bm{q}_{n},E)\delta_{\bm{n}',\bm{n}},
% \quad
% \mathbb{V}	=V(\bm{q}_{n},\bm{q}_{n'})\,.
% \end{eqnarray}
% The FV energy levels can be obtained by solving the equation 
% \be 
% \text{det}[\mathbb{G}^{-1}(E)-\mathbb{V}]=0.
% \ee
% One can introduce the modified Green function and potential matrices
% \begin{eqnarray}
% &\tilde{\mathbb{G}}^{-1}(E)	=E^{2}\mathbb{I}-\tilde{\mathbb{H}}_{0},\quad
% \tilde{\mathbb{V}}	=\frac{1}{L^{3}}\sqrt{\mathbb{N}}.\mathbb{V}.\sqrt{\mathbb{N}},\,
% \end{eqnarray}
% with
% \begin{align}
%  &   \tilde{\mathbb{H}}_{0}=[\omega_{1}(\bm{q}_{n})+\omega_{2}(\bm{q}_{n})]^{2}\delta_{\bm{n},\bm{n}'},\\
% &\mathbb{N}=\frac{\omega_{1}^{b}(\bm{q}_{n})+\omega_{2}^{b}(\bm{q}_{n})}{2\omega_{1}^{b}(\bm{q}_{n})\omega_{2}^{b}(\bm{q}_{n})}\delta_{\bm{n},\bm{n}'},
% \end{align}
%  and  identity matrix $\mathbb{I}$, so that the determinant equation to obtain the FV energy levels becomes $\text{det}[\tilde{\mathbb{G}}^{-1}(E)-\tilde{\mathbb{V}}]=0$. The solutions can be found by solving the eigenvector problem
%  \begin{equation}
%     (\mathbb{\tilde{H}}_{0}+\mathbb{\tilde{V}})\bm{v}=E^{2}\bm{v},~\label{eq:sm_hamilton_eq}
% \end{equation}
% where $\bm{v}$ is the eigenvector. 


% The plane wave basis with discrete momenta gives rise to a (reducible) representation of the corresponding point group. We can decompose this representation into irreps using the projection operator technique, which is discussed in detail in Ref.~\cite{Meng:2021uhz}. After reduction, the matrix $\mathbb{H}\equiv \tilde{\mathbb{H}}_0+ \tilde{\mathbb{V}}$ becomes block-diagonal, $\mathbb{H}=\text{diag}(\mathbb{H}^{\Gamma_1},\mathbb{H}^{\Gamma_2},...)$, where $\Gamma_i$ labels different irreps. For a specific irrep, one can obtain the FV energy levels by solving the eigenvalue problem of the sub-matrix, $\mathbb{H}^{\Gamma_i}\bm{v}=E^2\bm{v}$.

% In the above derivation, no partial wave expansion is performed. The usage of the plane wave basis is advantageous to include partial wave mixing effect arising from breaking of the rotation symmetry in a cubic box. In the context of moving two-body systems with unequal masses in the FV,  space inversion invariance is also broken,  resulting in a mixture of states with even and odd parities~\cite{Leskovec:2012gb,Doring:2012eu}. For example, for the states residing in the $A_2(1)$ irrep in Fig.~\ref{fig:E_FV} of the main text, the parity is not a good quantum number, since the energy levels in this irrep receive contributions from the $DD^*$ interactions both in $S$ and $P$ waves.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{figs/NN.pdf}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}



Our procedure can be formulated as a two-step process. In  step 1, we utilize our effective potential,   consisting of the OPE and a series of   contact interactions, to calculate the FV energy levels  both below and above the lhc from the condition that  the
determinant in the LSE vanishes.  
{ Technically, in our case, this amounts to solving the standard eigenvalue problem in the Hamiltonian approach, see Eq.~\eqref{eq:sm_hamilton_eq},
which is completely straightforward,  
 since  the off-shell $t$-channel potential entering Eq.~\eqref{eq:sm_hamilton_eq} only needs to be evaluated for real positive momenta. In this regime, the potential is completely analytic and free of  $t$-channel poles in the plane wave basis (or the $t$-channel lhc in the partial-wave basis).
}
Then, we adjust the low-energy constants   to achieve the best fit to the FV energy levels.  
In  step 2, we use the fully determined  effective potential, with all  low-energy 
constants  fixed  at  step 1,  to calculate the   infinite volume amplitude $T(E)$ from the LSE. 
How to deal with the last step technically is well known from phenomenology of two-body scattering at low-energies, e.g., from $NN$ scattering, where the effects from the lhc are included at the level of multi-pion exchanges, see, e.g., \cite{Epelbaum:2019kcf} for a recent review and \cite{Baru:2015ira,Baru:2016evv} for a related discussion.  The technique of solving the LSE in the infinite volume can be found, e.g. in the textbook~\cite{Landautxt}.
